Visual Manipulation with Legs

Animals use limbs for both locomotion and manipulation. We aim to equip quadruped robots with similar versatility. This work introduces a system that enables quadruped robots to interact with objects using their legs, inspired by non-prehensile manipulation. The system has two main components: a visual manipulation policy module and a loco-manipulator module. The visual manipulation policy, trained with reinforcement learning (RL) using point cloud observations and object-centric actions, decides how the leg should interact with the object. The loco-manipulator controller manages leg movements and body pose adjustments, based on impedance control and Model Predictive Control (MPC). Besides manipulating objects with a single leg, the system can select from the left or right leg based on critic maps and move objects to distant goals through base adjustment. Experiments evaluate the system on object pose alignment tasks in both simulation and the real world, demonstrating more versatile object manipulation skills with legs than previous work. Videos can be found at https://legged-manipulation.github.io/

==> limitation.tex <==
\section{Limitation}
\label{sec:Limitation}

While our system represents a notable exploration of using quadruped leg as a manipulator, it is not without its limitations. The use of an iPhone's lidar, for instance, introduces accuracy issues in point cloud observations due to distortion from reflective surfaces, impacting the inference of our learned policy \added{the registration result of RPM-nets. In the meantime, when facing object that are symmetry and lacking distinct feature, RPM-net can produce error in registration which leads to unexpected motion output from our policy.} Additionally, our reliance on MPC during training, although beneficial for sim-to-real transfer, faces challenges due to the absence of parallel processing for the Quadratic Programming (QP) problem. This limitation slows down training and hampers rapid policy development, \added{The current state estimator, which relies on the robot's internal IMU, is susceptible to translation and rotation errors. These errors can result in inaccuracies in motion parameters and contact location during execution. Additionally, the front-mounted camera's inability to capture the object's side point cloud further restricts the robot's action space.}


==> problem_statement.tex <==
\section{Task: Object Pose Alignment}	
\label{sec:Statement}


In this work, we focus on object pose alignment. The objective is to align an object's 6D pose with a given target pose, represented as a transformation relative to the current object pose. Using an observed object point cloud and the target transformation, the quadruped robot interacts with the object using its front legs to achieve alignment. By default, the left leg is used, except in the leg selection experiment (Section~\ref{legselection_benefits}). %We use single-step actions in this work. 


